Palette: Image-to-Image Diffusion Models

This paper develops a unified framework for image-to-image translation based on conditional diffusion models and evaluates this framework on four challenging image-to-image translation tasks, namely colorization, inpainting, uncropping, and JPEG restoration. Our simple implementation of image-to-image diffusion models outperforms strong GAN and regression baselines on all tasks, without task-specific hyper-parameter tuning, architecture customization, or any auxiliary loss or sophisticated new techniques needed. We uncover the impact of an L2 vs. L1 loss in the denoising diffusion objective on sample diversity, and demonstrate the importance of self-attention in the neural architecture through empirical studies. Importantly, we advocate a unified evaluation protocol based on ImageNet, with human evaluation and sample quality scores (FID, Inception Score, Classification Accuracy of a pre-trained ResNet-50, and Perceptual Distance against original images). We expect this standardized evaluation protocol to play a role in advancing image-to-image translation research. Finally, we show that a generalist, multi-task diffusion model performs as well or better than task-specific specialist counterparts. Check out https://diffusion-palette.github.io for an overview of the results.

==> main_figure.tex <==
% \begin{figure}[t]
% \vspace{-0.2cm}
% \small
% \begin{center}
% {\small
% \hspace*{-0.25cm}
% \begin{tabular}{@{}c@{\hspace{.15cm}}c@{\hspace{.095cm}}c@{\hspace{.095cm}}c@{}}
%      & Input & Output & Original \\
%      \raisebox{.4cm}{\rotatebox{90}{Colorization}} &
%      \frame{\includegraphics[width=.3\linewidth]{figs/main_figure/bw_bird0.jpg}} &
%      \frame{\includegraphics[width=.3\linewidth]{figs/main_figure/bw_bird1.jpg}} &
%      \frame{\includegraphics[width=.3\linewidth]{figs/main_figure/bw_bird2.jpg}} \\
%      \raisebox{.65cm}{\rotatebox{90}{Inpainting}} &
%      \frame{\includegraphics[width=.3\linewidth]{figs/main_figure/real_inp0.jpg}} &
%      \frame{\includegraphics[width=.3\linewidth]{figs/main_figure/real_inp1.jpg}} &
%      \frame{\includegraphics[width=.3\linewidth]{figs/main_figure/real_inp2.jpg}} \\
%      \raisebox{.5cm}{\rotatebox{90}{Uncropping}} &
%     %  \frame{\includegraphics[width=.3\linewidth]{figs/main_figure/uncrop0.jpg}} &
%     %  \frame{\includegraphics[width=.3\linewidth]{figs/main_figure/uncrop1.jpg}} &
%     %  \frame{\includegraphics[width=.3\linewidth]{figs/main_figure/uncrop2.jpg}} \\
%      \frame{\includegraphics[width=.3\linewidth]{figs/uncropping_comparison/22_src.jpeg}} &
%      \frame{\includegraphics[width=.3\linewidth]{figs/uncropping_comparison/22_palette.jpeg}} &
%      \frame{\includegraphics[width=.3\linewidth]{figs/uncropping_comparison/22_ref.jpeg}}\\
%      \raisebox{.7cm}{\rotatebox{90}{JPEG Res.}} &
%      \frame{\includegraphics[width=.3\linewidth]{figs/jpeg_comparison/3_src.png}} &
%      \frame{\includegraphics[width=.3\linewidth]{figs/jpeg_comparison/3_diffusion_l2.png}} &
%      \frame{\includegraphics[width=.3\linewidth]{figs/jpeg_comparison/3_ref.png}} \\       
%     %  \frame{\includegraphics[width=.24\linewidth]{figs/main_figure/real_inp0.jpg}} &
%     % \frame{\includegraphics[width=.24\linewidth]{}} & 
%     % \frame{\includegraphics[width=.24\linewidth]{}} \\[-0.01cm]
%     % % \frame{\includegraphics[width=.18\linewidth]{figs/main_figure/bw_room1.jpg} & 
%     %  \frame{\includegraphics[width=.24\linewidth]{figs/main_figure/bw_bird1.jpg}} & 
%     %  \frame{\includegraphics[width=.24\linewidth]{figs/main_figure/real_inp1.jpg}} &
%     %  \frame{\includegraphics[width=.24\linewidth]{figs/main_figure/uncrop1.jpg}}
%     %  &\frame{\includegraphics[width=.24\linewidth]{figs/main_figure/jpg1.jpg}} \\[-.01cm]
% \end{tabular}
% % \begin{tabular}{@{}c@{\hspace{.095cm}}c@{\hspace{.095cm}}c@{\hspace{.095cm}}c@{}}
% %     Colorization & Inpainting & Uncropping & de-JPEG \\
% %      \frame{\includegraphics[width=.24\linewidth]{figs/main_figure/bw_bird0.jpg}} & 
% %      \frame{\includegraphics[width=.24\linewidth]{figs/main_figure/real_inp0.jpg}} &
% %     \frame{\includegraphics[width=.24\linewidth]{figs/main_figure/uncrop0.jpg}} & 
% %     \frame{\includegraphics[width=.24\linewidth]{figs/main_figure/jpg0.jpg}} \\[-0.01cm]
% %     % \frame{\includegraphics[width=.18\linewidth]{figs/main_figure/bw_room1.jpg} & 
% %      \frame{\includegraphics[width=.24\linewidth]{figs/main_figure/bw_bird1.jpg}} & 
% %      \frame{\includegraphics[width=.24\linewidth]{figs/main_figure/real_inp1.jpg}} &
% %      \frame{\includegraphics[width=.24\linewidth]{figs/main_figure/uncrop1.jpg}}
% %      &\frame{\includegraphics[width=.24\linewidth]{figs/main_figure/jpg1.jpg}} \\[-.01cm]
% % \end{tabular}
% }
% \end{center}
% \vspace{-0.5cm}
% \caption{\model's results on four image-to-image translation tasks. No task-specific tuning or customization is used. %Inputs are on the top and outputs are below.
% %These results are from four Palette models trained on each task specifically, but without task-specific tuning or customization.
% %\chitwan{gray mask?} \huiwen{Added a black border to the inputs. We can add a black border to all the image to make it consistent. wdyt? \chitwan{+1 Good Idea}}
% % : colorization, inpainting, uncropping, and JPEG decompression.
% % \david{inpainting with stroke mask might be nicer here to appear less like uncrop.} \chitwan{Also, maybe let's not use Gaussian noise to denote the masked region, as it can be confusing?}
% % \david{definitely}
% % \huiwen{1) The outpainting examples in figure 7 look more impressive than the one in the teaser. What do you think? 2) The masks look different from masks in fig 5 and 6. Let's make them consistent?}
% % \mohammad{great points. we will have to remove faces too, so the inpainting example is no good?} \chitwan{Does the figure look good now?}
% }
% \vspace{-0.2cm}
% \label{fig:1}
% \end{figure}

% \begin{figure}[t]
% \vspace{-0.4cm}
% \small
% \begin{center}
% {\small
% \begin{tabular}{c@{\hspace{.095cm}}c@{\hspace{.095cm}}c@{\hspace{.095cm}}c@{\hspace{.095cm}}c}
%      & \multirow{2}{*}{Colorization} & \multirow{2}{*}{Inpainting} & \multirow{2}{*}{Uncropping} & JPEG \\
%      & & & & Decompression \\
%      \raisebox{0.7cm}{\rotatebox{90}{Input}} & 
%     % \frame{\includegraphics[width=.18\linewidth]{figs/main_figure/bw_room0.jpg} & 
%      \frame{\includegraphics[width=.23\linewidth]{figs/main_figure/bw_bird0.jpg}} & 
%      \frame{\includegraphics[width=.23\linewidth]{figs/main_figure/real_inp0.jpg}} &
%     \frame{\includegraphics[width=.23\linewidth]{figs/main_figure/uncrop0.jpg}} & 
%     \frame{\includegraphics[width=.23\linewidth]{figs/main_figure/jpg0.jpg}} \\[-0.01cm]
%      \raisebox{.6cm}{\rotatebox{90}{Output}} & 
%     % \frame{\includegraphics[width=.18\linewidth]{figs/main_figure/bw_room1.jpg} & 
%      \frame{\includegraphics[width=.23\linewidth]{figs/main_figure/bw_bird1.jpg}} & 
%      \frame{\includegraphics[width=.23\linewidth]{figs/main_figure/real_inp1.jpg}} &
%      \frame{\includegraphics[width=.23\linewidth]{figs/main_figure/uncrop1.jpg}}
%      &\frame{\includegraphics[width=.23\linewidth]{figs/main_figure/jpg1.jpg}} \\[-.01cm]
%      \raisebox{.35cm}{\rotatebox{90}{Reference}} &
%     % \frame{\includegraphics[width=.18\linewidth]{figs/main_figure/bw_room2.jpg} & 
%      \frame{\includegraphics[width=.23\linewidth]{figs/main_figure/bw_bird2.jpg}} & 
%      \frame{\includegraphics[width=.23\linewidth]{figs/main_figure/real_inp2.jpg}} &
%      \frame{\includegraphics[width=.23\linewidth]{figs/main_figure/uncrop2.jpg}}
%      &\frame{\includegraphics[width=.23\linewidth]{figs/main_figure/jpg2.jpg}} \\
% \end{tabular}
% }
% \end{center}
% \vspace{-0.5cm}
% \caption{Illustration of \model's performance on four image-to-image translation tasks, with input son top and outputs below.
% %\chitwan{gray mask?} \huiwen{Added a black border to the inputs. We can add a black border to all the image to make it consistent. wdyt? \chitwan{+1 Good Idea}}
% % : colorization, inpainting, uncropping, and JPEG decompression.
% % \david{inpainting with stroke mask might be nicer here to appear less like uncrop.} \chitwan{Also, maybe let's not use Gaussian noise to denote the masked region, as it can be confusing?}
% % \david{definitely}
% % \huiwen{1) The outpainting examples in figure 7 look more impressive than the one in the teaser. What do you think? 2) The masks look different from masks in fig 5 and 6. Let's make them consistent?}
% % \mohammad{great points. we will have to remove faces too, so the inpainting example is no good?} \chitwan{Does the figure look good now?}
% }
% \vspace{-0.2cm}
% \label{fig:1}
% \end{figure}

